S2-Attention: Hardware-Aware Context Sharding Among Attention Heads

Sparse attention, which selectively attends to a subset of tokens in the context was supposed to be efficient. However, its theoretical reduction in FLOPs has rarely translated into wall-clock speed-up over its dense attention counterparts due to the lack of hardware-aware optimizations like FlashAttention. Meanwhile, it remains unclear whether sparse attention can maintain the model's quality at a scale of today's large language models (LLMs) and how. This paper presents Sparsely-Sharded(S2) Attention, a Triton library that provides kernel optimization for sparse attention customizable at both per-head and per-context-range levels. S2-Attention enables the exploration of novel and high-performance sparse attention techniques, which we demonstrate through extensive ablations across a wide range of sparse attention designs at various model scales. From these insights, we present several basic guidelines to design sparse attention that can achieve not only practical efficiency improvements, but also strong downstream performance. To achieve high parallelization and optimized memory IO, sparse attention should shard the context heterogeneously across attention heads, where each head attends to a different subset of tokens while collectively covering the full context. Meanwhile, we find hybrid architectures combining sparse and dense attention particularly beneficial in practice. S2-Attention achieves wall-clock speedup of 8.79X, 15.87X, 25.3X compared to the strong FlashAttention-2 baseline with strong downstream performance on-par with full attention and perfect retrieval performance at a 128k context length. At inference, for 7B models, our model, with the help of our S2-Attention kernel, achieves 4.5x speed-up compared to dense counterparts. S2-Attention is released with easy-to-customize APIs for direct usage in Megatron and vLLM.

==> inputs/impact.tex <==
This paper aims to provide a easy-to-user kernel library for researchers to better explore sparse attention, as well as sharing insights into making sparse attention more practically sound in real-world deployment.
There are many potential societal consequences of our work, none which we feel must be specifically highlighted here.

==> inputs/intro.tex <==
\hao{general thoughts on the intro:
\begin{itemize}
    \item (major) we are not giving enough credit to prev sparse attn works. the current narrative reads that, based on the sparsity observations, we, independently of prev works, propose a new sparse attn framework that does better than previous ones. this can invite some criticisms. first, if the major contribution is framed as a new sparse architecture, it should be compared to Child 19, Ho 19, Beltagy, and many baselines to support the statement that ours does better than these works, which i don't think we have included in the exps nor do i think it is worth doing. this is also risky if we have reviewers tha are very picky about `novelty' since sparse attn is a widely-studied topic.
    (repeating my prev comment) an alternative approach would be to fully acknowledge previous sprase attn, say the benefits of sparse attn have been fully proven, which inspires us to further explore it. we, based on insights into the hardware and mlsys, propose a new sparse attn architecture that is much more compatible w/ hardware and mlsys infrastructure and scalable to large model/data/context lengths. we, for the first time, also provide the cuda kernel not only for our model, but alto for many other sparse attn variants, which would incentivize future research
    \item our algo being designed in a hardware-aware manner is not emphasized enough. i like it that we are comparing to flash attn; given this, we should highlight that our algo is not only inspired by sparity observation, but also what would actually be efficient in practice on gpus
    \item the paragraphs starting with "In this way" and "In this paper, we provide" can be swapped and trimmed for a better flow---we introduce \ours right after its three design principles, and then talk about its benefits.
    \item we jump between training vs. inference, long context vs. any context when talk about overhead and saving, which makes it very confusing to follow. my understanding is that \ours brings saving for short context too (fig 1(a)). this makes the opening sent of second paragraph inappropriate.
    \item i'm not sure we need the two examples about training and serving llama2 70b--it is well known that pretraining is expensive and we don't need to educate the readers; serving a 70b bsz 16 model w/ 43gb memory, basically a mid-range gpu, does not look bad at all.
\end{itemize}
}

Transformer-based large language models~\citep{openai2023gpt4,touvron2023llama} have brought about revolutionary opportunities to research and applications. 
% These models advance various difficult tasks and user-scenarios like general chat assistant and open domain question answering to an unprecedented level.
The remarkable success of these models across diverse applications underscores the pressing need for training and serving these models economically.
%discuss training and inference cost: kv(memory), tiling(IO), and flops(N**2).
% self attention higher percentage total time as model scales up
% training needs extra backward cost example, forward can use kv cache example

%The core of the transformer architecture is the self-attention mechanism. 
Self-attention, the core of the transformer architecture, incurrs quadratic time and memory complexity in the context lengths, making it prohibitively expensive to scale to longer context.
\hao{agree w/ Suyu's comment, this reads like \ours is mainly useful for long contexts, but by figure 1, it also brings savings for short ones.}
% The issue becomes more severe with the model size increase, as the self-attention modules even accounts for a higher percentage of total execution time \cite{flash}.
For example, with a 4K context length, training Llama 2 70b on 2 trillion tokens \cite{touvron2023llama} needs 23 days to finish with 2048 A100 GPUs \cite{cost}, which is estimated to cost 2 million dollars.
\begin{figure*}[h]
\begin{subfigure}[]{0.55\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/attn_bench_70B.pdf}
    \caption{Speedup over FlashAttention-2. \hao{suggest changing this to throughput in tokens/s, so that higher the better. it is also a more common metric for training efficiency}
    \hao{specify this is training}
    \hao{since we are claiming both training and inference, maybe clarify that inference speedup is the same as the left-hand side}
    \hao{do we also save memory}}
\label{fig:attn_bench}
\end{subfigure}
\begin{subfigure}[]{0.45\textwidth}
     \centering
     \includegraphics[width=\textwidth]{Figures/needle_heatmap_32768.pdf}
     \caption{Needle in a haystack evaluation.}
     \label{subfig:helpeval}
\end{subfigure}
\caption{Training Efficiency and long-context analysis of S2-Attention.}
\end{figure*}

During inference, 
previously computed key and value vectors (KV Cache) are stored to avoid recomputation, substantially increasing the memory overhead.
% the forward pass of LLMs typically involves storing the previously computed key and value vectors (KV Cache) to avoid recomputing.  
% Known as \emph{KV Cache}, the strategy improves the generation speed but would incur even larger GPU memory footprint linear to the product of model size and total sequence length \cite{fastgen}.
For instance, serving Llama 2 70b requires a staggering 43 GB of KV cache with a batch size of 16 and a context length of 2K. 
% When the memory usage goes beyond the GPU memory capacity, the KV Cache needs to be offloaded to CPU memory or even to NVMe memory~\citep{Aminabadi2022DeepSpeedIE,Sheng2023HighthroughputGI}, which would introduce significant overhead.
% So to secure the research and product competition, companies have to costly deploy excessive number of accelerators.

\hao{the benefits of sparsity are not clearly laid out.
at least the following points should be covered:
(1) compared to alternatives such as state based models, it is largely compatible w/ attention and requires minimal changes to the architecture.
(2) it retains the performance while greatly reduce the memory and time overhead for both training and inference
(3) (rather than the database analogy) in terms hardware, it is friendly to current software and hardware infrastructure and can equally benefit from their advances as the regular attn.
}
We aim to improve the training and inference efficiency of LLMs.
We start from the observation of the inherent sparsity of transformers \citep{retrievalhead, inductionhead, fastgen}. 
As illustrated in Figure \ref{fig:obs}, despite densely trained, the majority of attention mass still concentrates on a few tokens:
for most cases, fewer than $1\%$ tokens receive over $95\%$ attention mass.
% can be recalled with less than $1\%$ tokens. 
Also, different attention heads could have dynamically different attention mass distribution patterns. 
% Inspired by the observation, we want to examine how would applying the sparsity observed in inference to training affect the model quality.
% Then the research question is, 
\hao{the following couple of sents go back and forth between inference and training, which read very confusing. }
As inference works with a sparse subset of contexts for each head, can we accelerate training by enforcing this sparsity on each head?
More specifically, we want to examine how to maintain the model quality while maximally reducing the context load of every attention head \textbf{in training}.
From a hardware perspective, as each attention head is processed independently by a distinct thread block, assigning a subset of the context to each thread block is similar to the sharding concept in database. \hao{repeating my earlier comments---sparse attn is already well-known among the audience we are targeting, while database techniques are not. i'm not sure this database analogy would help reader to follow our motivation}  
% Previous attempts \citep{sparsetransformer,axial,bigbird} overlooks  
Thus, we design Sparsely-Sharded (S2) Attention built on three key premises \hao{these are not premises per say, but more of a set of intuitions and design principles}:

\begin{figure}[t!]
\includegraphics[width=\textwidth]{Figures/s2visual.pdf}
\caption{Illustration of \ours with four attention heads on a hypothetical GPU with 4 thread blocks. Each attention head is allocated with a shard of the context.}
\label{fig:pipeline}
\end{figure}

% to reduce load while maintaining context
P1: In training, we can get equivalent model quality while allocating only a partition of the context to each attention head, as long as \textbf{the union of all the shards equals the complete context}.
%\hao{we need to cite: %https://arxiv.org/pdf/1904.10509 and https://arxiv.org/pdf/1904.10509}

% to better mimic the diverse patterns among heads?
P2: Following P1, attention heads should attend to diverse shards. Under the same compute budget, models trained with \textbf{heterogeneous sparsity pattern} on attention heads would have a better quality over those trained with homogeneous sparsity pattern. 

P3: Dense attention layers \hao{do we mean full context? dense layers usually mean ffns in transformer contexts }at certain point are necessary for preserving model quality. 

In this way, \ours can be trained with significant fewer FLOPs while maintaining the model quality, including long context capabilities, compared to those trained with default \hao{canonical} attention.
Compared to previous sparsity method \citep{sparsetransformer,axial,bigbird}, sharding the context among numerous attention head can achieve higher sparsity per head, while explicitly maintaining the full context.
Also, the heterogeneous assignment could better utilize the multi-head expressiveness compared to previous homogeneous designs. 
During serving, \ours can then take KV Cache saving as a free meal while having a better quality guarantee, as each attention head is originally trained on reduced contexts.

In this paper, we provide an instantiation of \ours that satisfies all the arguments.
We first chunk the sequence of tokens into blocks.
For an attention head $h$, it only attends to the blocks that are adjacent to the current token, and blocks whose ids are divisible by a stride after offset by $h$ . 
A larger stride means each attention head receives a smaller, and more sparse shard.
The stride size is between 1 and number of attention head, which secure the union can preserve full context.
Lastly, we keep the first two dense layers dense while the rest of layers sparse, as we find it's crucial to maintain the initial layers intact.

% may need to double check task types and prompt length
We validate the effectiveness of \ours by evaluating the model quality on a wide range of tasks covering context retrieval, common sense reasoning, and question answering. 
Across benchmarks, \ours achieves on par, or even better performance compared to densely trained models. 
For training efficiency benefit, compared to Flash-Attention 2, \ours can achieve as much as 8.8X wall-clock speed-up at 128K sequence length for 1.3B model. 
The boost increases as the model and context length scales up. 
On a 70B model with 64 heads, \ours can bring 25.3X speed-up.
For inference speed-up, \ours can achieves up to 12X speed up over FlashAttention-2 on a 1M context window.
Lastly, we back \ours with an optimized kernel library, \repo, designed to be a plug-in-and-play replacement of the popular FlashAttnetion-2 and PyTorch SPDA used in most modern training frameworks. 
It allows users to freely customized the interested pattern they want to study in both training and inference. 
Lastly, we've integrated \repo into vLLM for easy adoption in serving.




==> inputs/limitations.tex <==
We've shown that we can get almost the same model performance with sparse sharding,
there are some obvious limitation worth to be outlined. \\

We pretrained a relatively small model from scratch with 300B web-heavy data,
regardless it is with dense attention or \ours, is relative weak for evaluation,
due to both the model capacity and training horizon. It will be better to 
experiment with a larger model and longer horizon. However, the cost is prohibitive.
However, our message at the current scale of model and data is still clear,
attention does not need to be dense, and \ours attention can achieve similar performance
with much less computation.


==> inputs/method.tex <==
\label{sec:method}
\subsection{Preliminary}
In this section, we first present  formulation of the context sharding process for Sparsely Sharded Attention (\oursshort).
Then we discuss context-sharding policies we designed to instantiate \oursshort.
Lastly, we analyze why \ours can achieve significant wall-clock speed-up for both training and inference.
\subsection{Context Sharding}
Let \( \mathcal{X} = \{x_1, x_2, \dots, x_N\} \) be the input sequence where \( N \) is the length of the sequence,
\( \mathcal{H} = \{h_1, h_2, \dots, h_K\} \), where \( K \) is the number of attention heads.
Each attention head \( h_k \) is associated with a shard \( S_k \) of the sequence \( \mathcal{X} \), determined by a context sharding policy $f$. 
The  policy can be viewed as a mapping function \( f: \mathcal{H} \to 2^{\mathcal{X}} \), where \( 2^{\mathcal{X}} \) is the power set of \( \mathcal{X} \). 
Each head receives a subset of the sequence elements: \( f(h_k) = S_k\).


We design the sharding process to meet the following properties:
\begin{enumerate}
  \item \textbf{The union of all the shards equals the full context.} Namely, each element \( x_i \) in \( \mathcal{X} \) must be assigned to at least one shard. Formally, this can be expressed as:
  \[
  \bigcup_{k=1}^{K} S_k = \mathcal{X}
  \]
  \item \textbf{Different attention heads receive heterogeneous context shards.} At least two heads should receive different subsets of \( \mathcal{X} \). Specifically:
  \[
  \exists i, j \in \{1, \dots, K\}, \, i \neq j : S_i \neq S_j
  \]
  \item \textbf{Initial layers should receive full context for optimal performances.} For simplicity, we set the initial two layers to be dense and sparsely shared contexts among the rest layers.
% \[
%   \exists k \in \{1, \dots, K\} : S_k = \mathcal{X}
%   \]
%   This constraint may be relaxed.
\end{enumerate}

\subsection{Context Sharding Policy Choices}
From our experiments in Figure \ref{fig:obs} and previous studies \citep{fastgen,retrievalhead}, we summarize 6 basic attention patterns in trained transformers detailed in Section \ref{sec:observation}.
As we found the \textbf{Local} pattern is most common across attention heads, we first ensure each shard includes local context.
For contexts out of this local window, termed as remote context, we would like the sharding policy to cover the \textbf{Attention Sink}, \textbf{Middle Spikes} and their hybrid combinations \cite{fastgen}.

To capture the huge combinations while maintaining sparsity, we take advantage of the inherent  expressiveness in the \textbf{multi-head} architecture.
Each attention head is assigned with strided partitions of the remote contexts, \textbf{with the starting points of these partitions uniquely offset by the index of the corresponding head.}
The heterogeneous assignment allows for a nuanced and scalable coverage of remote contexts.
By combining the two designs, we introduce a heterogeneous strided sharding policy as formulated below.
% To provide a general coverage of all the patterns, we design a heterogeneous local-stride pattern as detailed below.\\
\subsection{Heterogeneous Strided Sharding}

\textbf{KV-cache efficient sharding has a vertical pattern.}  For any $l \geq 1$ and $j \geq i$, we say a sharding $S$ is KV cache efficient if $k_i, v_i$ is attended by $q_{j+l}$, then it must be also attended by $q_j$. Otherwise, $k_i, v_i$ has to be stored at token $j$ for generating token $j+l$, but not used to generate token $j$. In this case, we can just let $q_j$ also attend to $k_i, v_i$ without additional memory for KV cache. However, some tokens in KV cache can be dropped after generating certain tokens. This also means that the sharding $S$ should be based on absolute token positions. From the aspect of 2-dimension attention mask as shown in Figure 2, the tokens attended to (K/V), must be a single line segment starting from the diagonal line and ending somewhere after. This means that the sharding must have a vertical pattern.

\begin{figure}[!h]
    \centering
    \includegraphics[width=0.45\linewidth]{Figures/ok_pattern.pdf}
    \includegraphics[width=0.45\linewidth]{Figures/bad_pattern.pdf}
    \caption{Left: KV-cache efficient sharding. Right: sharding that is not KV-cache efficient since token 2 is not attended by tokens 2 - 11, but needs to be stored at token 12 to generate token 13 and onward, i.e., the first vertical green line does not start from the diagonal line. The upper right corner is masked due to causal attention.}
    \label{fig:enter-label}
\end{figure}

\textbf{Vertical pattern with one fixed stride and a local window.} 
From the KV-cache efficiency perspective as discussed above, the attention pattern should follow a vertical pattern. Given the important of adjacency of natural language, a certain local window should also be included. A simple pattern that meets these criteria is a pattern with fixed vertical stride and a local window.   

For a transformer with $H$ heads, given a sequence of $N$ tokens, we first chunk context into a list of blocks of size $S$, which gives us $B=ceil(N/S)$ blocks.
We use $q_i$ and $k_i$ to denote the query block and key block index.
Note that $q_i$ corresponds to the $i$ th indexed block, instead of the $i$ th token, and one block includes $S$ tokens.

Among the total $B$ blocks, We take the most recent $N_{l}$ blocks as local blocks and set the rest as remote blocks.
Since local blocks are more frequently attended, we use different stride sizes for local and remote blocks for fine-grained context modeling.
Denote the local stride as $v_l$ and remote stride as $v_r$.
For simplicity, we use full attention for local blocks by setting $v_l=1$, since local blocks only accounts for a small portion of the total context and brings negligible change to the overall efficiency.
In practice, $v_r$ is set to be a factor number of attention heads to satisfy the ``union as full context'' constraint.
% For vertical stride of $v_1, v_2$ where $v_2\, \%\, v_1 = 0$, the local-stride block pattern looks like
For each head $h \in \{1, ..., H\}$, we set a unique position offset $o_h$. For simplicity, we set $o_h = h$ here, which means the offset of each head equals its head index.

Then for each head $h$, its block attention mask $M^h$ in $B \times B$ dimension is as follows:
% \[
% I(b_k) = 
% \begin{cases} 
%     1 & \text{if } (b_k - z^h_1) \mod v_1 = 0 \text{ and } b_q - b_k < N_1, \\
%     1 & \text{if } (b_k - z^h_2) \mod v_2 = 0 \text{ and } b_q - b_k \geq N_1, \\
%     0 & \text{otherwise}
% \end{cases}
% \]
\begin{equation} \label{local-stride-hetero}
M^h_{i,j} = 
\left\{
\begin{array}{ll}
    1 & q_i - k_j < N_l,  \\
    1 &  (k_j - o_h) \in v_r \mathbb{Z}_{\geq 0}\,\&\, q_i - k_j \in [N_l, B) \\
    0 & \text{otherwise},
\end{array}
\right. 
\end{equation}

where $x \in m\mathbb{Z}_{\geq 0}$ mean $x$  is 0 or a positive multiple of $m$.

The first constraint determines the shards within the local window. 
The second constraint controls what shard each head attends to outside the local window. Note that if the distance is beyond $B$, the attention is dropped, thus extends similar to a sliding window.
As an example, setting \( B = 8, N_l = 2, v_l = 1, v_r = 3, o_h = h\) will give us the sharding as presented in the left part of Figure \ref{fig:exp_main}. 
\( B = 8, N_l = 3, v_l = 2, v_r = 3, o_h = h\) will give us the right part of Figure \ref{fig:exp_main}.
\begin{figure}[h]
\centering
\includegraphics[width=0.85\textwidth]{Figures/localstride.pdf}
\caption{Example Sparsity Patterns.}
\label{fig:exp_main}
\end{figure}
% \begin{equation} \label{local-stride-hetero}
% I(b_k) = 
% \left\{
% \begin{array}{ll}
%     \delta_{(b_k - z^h_1)\, \%\, v_1 = 0} &  \text{if } b_q - b_k < N_1  \\
%     \delta_{(b_k - z^h_2) \, \%\, v_2 = 0} &  \text{if } b_q - b_k \geq N_1 \\
% \end{array}
% \right. 
% \end{equation}

% Note that, the $v_1$, $v_2$ regions are determined by relative block position (block chunking are fixed on absolute position), the masking at each region is indeed determined by the absolute position. This is critical, otherwise, one has to save all KV caches for all blocks when decoding one token after another at inference time.

% We enforce  $v_2 \% v_1 = 0$ here for KV cache saving at inference, as otherwise, one has to keep all the full KV for all blocks.  
% %TODO make this more clear and intuitional @Eric
% With the constraint, as KV grows from the region of $v_1$ stride to the region of $v_2$ stride, the $v_1$ KV cache can be naturally truncated.
% In this way, we can reduce the KV cache to a factor of $v_2 / v_1$.

We pick this neat instantiation but the formulation is quite general.
% It can be easily extended to a series of vertical strides of ${v1, v_2, ..., v_N}$, where $v_{i+1} \% v_{i}  = 0$. 
The constraints can also be met by choosing different offset $o_h$, or different vertical stride $v_i$, or local attention window size $N_l$ for each head, which are all supported by our library. 


\textbf{Vertical pattern with multiple fixed strides and a local window.}
This local-stride pattern can be easily extended to have multiple strides in different remote blocks. With blocks $N_l < N_{r_1} < N_{r_2} < B$, and $v_{r_1} < v_{r_2}$, we define block attention mask as

\begin{equation} \label{multi-stride-hetero}
M^h_{i,j} = 
\left\{
\begin{array}{llll}
    1 & q_i - k_j \in [0, N_l), &&  \\
    1 &   q_i - k_j \in [N_l, N_{r_1}) & \& & (k_j - o^1_h) \in v_{r_1}\mathbb{Z}_{\geq 0},\\
    1 &   q_i - k_j \in [N_{r_2}, B) & \& & (k_j - o^2_h) \in v_{r_2}\mathbb{Z}_{\geq 0}, \\
    0 & \text{otherwise}.
\end{array}
\right. 
\end{equation}

To ensure that $M_{i,j}^h$ is KV-cache efficient, we requires that
$v_{r_2} \in v_{r_1}\mathbb{Z}_{\geq 0}$ and $(o^2_h - o^1_h) \in v_{r_1}\mathbb{Z}_{\geq 0}$.

% But here for notation simplicity, we assume $v_i$ are the same for all heads, but the offsets $z_h$ are head specific.

% If the block mask pattern designed in \ref{local-stride} is exactly the same for all heads, we said the heads are homogeneous, other we call the heads heterogeneous.

% If $z^h_i$ is the same for all $h$ for a given $i$, the heads are homogeneous. 
% In practice, we choose $z_i^h=\max(1, v_i // H)$.

% Assuming $v_1 = 1$ (local sliding window) and $N2$ is the sequence length. If $v_2 \le H $, in the heterogeneous case, all tokens are attended to at $H / v_2$ heads, instead of all heads as in dense. While in homogeneous case, some tokens will be completely skipped if it not beyond the local region.

%  In our experiments, we choose different offsets $z_h$ for each head, while keeping vertical stride and local window constant for the comparison between homogeneous and heterogeneous patterns, as the sparsity levels are the same in both cases. 
% However, choosing different vertical strides and local window are something also very interesting, especial in the case where we have some heads that are dense while others are sparse. 
% We leave these experiments to the future.


% \begin{figure}[!h]
%     \centering
%     \includegraphics[scale=0.4]{./Figures/homo-vs-hetero.png}
%     \caption{Homogeneous sparse pattern (all heads attend to the same blocks) vs Heterogeneous sparse pattern (different heads can attend to different blocks of tokens.}
%     \label{fig:hetero}
% \end{figure}



% \subsection{Hierachical strides}

% \subsection{Interact with Group Query Attention}

% Grouped attention is getting common in LLM training as it reduces key-value cache by $G$ folds if each key-value pairs are shared by $G$ query heads. 
% However, it has some interesting interaction with the sparse pattern on the vertical stride region. 
% From KV cache saving standpoint, it is better to have the $q_{ig}, g\in{1, ..., G}$ attend the same blocks of $k_i$, i.e., homogeneous patterns within each group, as in this way, the KV cache on the vertical stride region will be reduced by $V$ fold. 
% Between the groups, we have have different patterns. 

% However from the perspective that it is better to attend to different blocks for different heads, it is also interest to have different patterns within the same attention group.

\subsection{Training and Inference Advantages}
With the formulation of \ours, we can achieve significant FLOPs reduction in training.
To train a default self-attention layer, the total FLOPs needed is $O(TN)$, where $T$ is the number of tokens to train, $N$ is the max sequence length.
% $H$ is the number of attention head, and $D$ is the head dimension.
When using \ours, in case where $v_l=1$, we have a dense local window of $L$ tokens, and the vertical stride $v_r=v$ for the remote context.
For each attention head, $L + (N-L)/v$ is number of tokens attention to, i.e. the dense equivalent sequence length.
Then the total FLOPS reduced from $O(TN)$ to $O(T(L + (N-L)/v)$ at an attention layer. 
For a 1.3B Llama-like model with 16 attention heads, 
trained on 8192 sequence length, set $L = 64$ and $v = 16$ will generate a 14.32X FLOPs reduction.
As the stride $v$ is bounded by the number of heads for the union constraint, we can have larger v choices as the model size increases, which will further boost the reduction.
It can be derived that the upper bound of the speed-up grows linearly with the number of attention heads.
For example, for a 70B model with 64 attention heads, \ours can generate 42.89X reduction.

During inference, the prompt prefilling stage has the same FLOPs saving as the forward pass in training.
In the decoding phase, despite the FLOPs saving, \ours will have extra memory footprint reduction.
As each attention head is processed in one Streaming Multiprocessor(SM), skipping the blocks outside the shard of a given head can thus reduce the memory usage, which further boosts throughput. 

% \subsection{On-the-fly Adaptive Inference}
% To further boost the inference performance, we study the sparsity distribution of the models trained with \ours.
% As shown in Figure \ref{fig:obs}, the attention score distribution still shows a dynamically sparse pattern among attention heads.
% The observation motivate us to further harvesting such structure.
\subsection{System Implementation}
% In this section, we discuss our kernel optimization to achieve actual wall-clock speed-up. 
% \textbf{TODO: may need to discuss details making the sparse mask fast and memory/IO efficient.}
% The original OpenAI implementation is not based on the idea of fused attention proposed by flash attention. The blocksparse attention in the Flash attention paper is very efficient, but we've found it difficult to use it.
Our \ours training kernel is developed upon the Triton flash attention code. 
We've compared it to the CUDA version of FlashAttention-2. 
It accepts a tensor specifying the per head sparsity pattern on a shard level. 
The underline algorithm turns the sparse matrix to compressed sparse row (CSR) format as input, which contains k shard indices for each q shard, then scan over the k shard indices to do the FlashAttention in a thread block. 
We see that when vertical stride is set to 1, e.g., normal dense attention, the latency is comparable to the original Triton flash attention. 
Compared to the CUDA version of Flash Attention 2, the forward pass has similar latency while the backward pass lags slightly. 
When the vertical stride increases, the performance increase almost linearly as shown in Figure \ref{fig:dsplit}. 
The memory usage in S2-attention is the same as FlashAttention-2 in training regardless of the vertical stride. 
However at inference, during the decoding phase, the KV cache is about $1/v$ of a dense attention if local window is considerably small compared to the current sequence length.

\textbf{Block merging and splitting} The sparse block size could potentially be small to avoid long skip in the attention pattern, but kernel block size are usually required to be much larger to increase GPU efficiency.  We merge the sparse blocks having same K/V blocks but different Q blocks. Thanks to the efficient KV cache insight above, we can easily distinguish between dense blocks and partially dense block at loading and compute time, by passing the number of blocks merged in a mega block. Thanks to this, we are able to support sparse block size as small as 16.

If the sparse block size is larger than the best kernel block size, we simply break the larger sparse block to a few of smaller blocks that are optimal for GPU.

\textbf{D-split} Both the CUDA version and the Triton version of flash attention load the whole head dimension(D) at once to SRAM, which is intuitive as the whole vector is needed to compute the attention scores. 
However, in our experiment, we found that split at the D dimension in many cases is beneficial. 
We suspect that this is because D-split reduce SRAM usage and enable a larger degree of software pipelining. 
Interestingly, we also find that with shard size of 64, D-split only helps when head dimension is 128, the most commonly used case, while has no additional benefit when head dimension is 64 or 256.
We suspect that this is due to under-tuned hyper-parameters like kernel block sizes.
% \\
% \textbf{NOTE} \\
% \textit{should we mention here or in limitation? 
% I believe we can make it better with D-split, but requires addition work.
% }

\begin{algorithm}
\caption{Scratch of D-split at the forward pass in a thread block. See \cite{flash2} for more detail}\label{alg:cap}
\begin{algorithmic}
\State \textbf{Init} SRAM $b, p, q_0, q_1, o_1, o_2$
\State \textbf{Load} $q_0 \gets q[..., :D/2]$, $q_1 \gets q[..., D/2:]$
\For{\texttt{j in attn\_shard\_indices}}
    \State \textbf{Load} $b \gets k_0^j$
    \State $p \gets q_0@b$
    \State \textbf{Load} $b \gets k_1^j$
    \State $p \gets p + q_1@b$
    \State $p \gets \mathbf{softmax}(p)$
    \State \textbf{Load} $b \gets v_0^j$
    \State $o_1 = update(o_1, p@b)$
    \State \textbf{Load} $b \gets v_1^j$
    \State $o_2 = update(o_2, p@b)$
\EndFor
\end{algorithmic}
\end{algorithm}
\begin{figure}[t!h!]
\centering
\includegraphics[width=0.8\textwidth]{Figures/latency_split.pdf}
\caption{Left: Comparison between dense and S2-attention with different sparsity. All experiment use (batch, heads, head\_dim) = (4, 16, 128) on A100 80GB-SXM. Right: Impact of D-split. All experiments use (batch, heads, head\_dim) = (4, 16, 128) on A100 80GB-SXM. We see D-Split=2 consistently outperforms D-Split=1 in most implementation of flash attention on the forward pass. However. the impact on the backward pass is negligible.}
\label{fig:efficiency}
\end{figure}
% \begin{figure}[!h]
%     \centering
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[scale=0.23]{Figures/fwd_algorihtm.pdf}
%     \includegraphics[scale=0.23]{Figures/bwd_algorihtm.pdf}
%     \caption{Comparison between dense and S2-attention with different sparsity. All experiment use (batch, heads, head\_dim) = (4, 16, 128) on A100 80GB-SXM.}
%     \end{subfigure}
%     \begin{subfigure}{0.48\textwidth}
%     \includegraphics[scale=0.23]{Figures/fwd_all_vert_dsplit_0_vs_1.pdf}
%     \includegraphics[scale=0.23]{Figures/bwd_all_vert_dsplit_0_vs_1.pdf}
%     \caption{Impact of D-split. All experiment use (batch, heads, head\_dim) = (4, 16, 128) on A100 80GB-SXM. We see D-Split=2 consistently outperforms D-Split=1 in most implementation of flash attention on the forward pass. However. the impact on the backward pass is negligible. }
%     \end{subfigure}
%     \label{fig:kernel}
% \end{figure}

% \section{Experiments}
% \label{sec:exp}

% \subsection{Experiment setup}

% \subsection{Figures}
% % \lipsum[10] 
% % See Figure \ref{fig:fig1}. Here is how you add footnotes. \footnote{Sample of the first footnote.}
% % \lipsum[11] 

% \begin{figure}[!h]
%   \centering
%   % \fbox{\rule[-.5cm]{4cm}{4cm} \rule[-.5cm]{4cm}{0cm}}
%   \includegraphics[scale=0.1]{Figures/loss-time.png}
%   \caption{Validation losses and training times (include checkpoint of times) of a 1.3B model(24 layers, 2048hidden, 24 layers) on 128 A100-40G SXM GPUs across 16 nodes with Infinite Band. Convert to Flash attn2 by the FLOPs reported in FlashAttention-2 paper which is 82.7hours or 3day11h.  \textbf{!!TODO: find log and remove the checkpointing time.}}
%   \label{fig:fig1}
% \end{figure}

% \textbf{TODO: get an estimate on training time with 32k/64k if not OOM swith TP=1.}

% \subsection{Tables}
% \lipsum[12]
% See awesome Table~\ref{tab:table}.

% \begin{table}
%  \caption{Sample table title}
%   \centering
%   \begin{tabular}{lll}
%     \toprule
%     \multicolumn{2}{c}{Part}                   \\
%     \cmidrule(r){1-2}
%     Name     & Description     & Size ($\mu$m) \\
%     \midrule
%     Dendrite & Input terminal  & $\sim$100     \\
%     Axon     & Output terminal & $\sim$10      \\
%     Soma     & Cell body       & up to $10^6$  \\
%     \bottomrule
%   \end{tabular}
%   \label{tab:table}
% \end{table}

% \subsection{Lists}
% \begin{itemize}
% \item Lorem ipsum dolor sit amet
% \item consectetur adipiscing elit. 
% \item Aliquam dignissim blandit est, in dictum tortor gravida eget. In ac rutrum magna.
% \end{itemize}


==> inputs/observation.tex <==
\label{sec:observation}
\begin{figure}[t!h!]
\includegraphics[width=\textwidth]{Figures/merge.pdf}
\caption{Left: Attention mass sparsity in different heads during decoding the same sequence. Right: Sparsity in different layers. Except for the bottom layer, all other layers display significant attention sparsity. Experiments are done on Llama3-8B with different task prompts, including needle retrieval, summarization and math.}
\label{fig:obs}
\end{figure}
In this section, we present an empirical study to see what each attention head actually attends to at inference time.
We conduct experiments on Llama-3 8B \citep{meta2024introducing} using a 2048 context length.
We first start with the overall layer by layer pattern, then showcase specific sparsity patterns we find.

\textbf{Scattered Distribution in Initial Layers}.
In the initial layers, attention score is generally uniform for all heads. 
We call this pattern \textbf{Uniform Scatter}, which is illustrated at the right of Figure~\ref{fig:obs}.
Such pattern suggests the model does not heavily prioritize any specific part of the input.
Thus, it's risky to reduce the context when the head show such patterns.
Intuitively, these attention layers should be kept dense. 

\textbf{Sparse Patterns in Middle Layers}.
As we move deeper into the network, the attention mechanisms exhibit a marked departure from uniformity.
We start with identifying simpler patterns.
\textbf{Attention Sink} \cite{sink} and \textbf{Locality} can be seen in a small subset of heads.
For these heads, nearly all attention probability concentrate on the first few tokens or tokens adjacent to the current position, as shown in the upper left and upper right of Figure~\ref{fig:obs}.

\textbf{Middle Spikes}, as shown in Figure~\ref{fig:obs}, can also be identified in a few heads.
This pattern puts significant probability mass on a few tokens that are in the middle of the context.

However, the vast majority of attention heads actually show a more complex hybrid pattern that could be decomposed into patterns mentioned above. 
For example, hybrids like Attention Sink + Local, or Attention Sink + Middle Spikes + Local are 
the most prevalent patterns, which is also demonstrated in \cite{fastgen,attnpattern}.

% \textbf{Hybrid Patterns in Final Layers}
% We can observe a more hybrid and scattered pattern in the final layers. 
% Each head can have a diverse array of attention strategies, which suggests its role as a comprehensive integrative mechanism over earlier layers.
% In other words, the attention is denser compared to earlier layers.

% In short, we find the attention probability is sparse in most cases, yet the actual attention pattern is quite diverse and complex among attention head.
From the observation, we can conclude that (1) individual attention heads do not necessarily take the full context to function, (2) the actual context needed by different heads can be quite different, and (3) the initial attention layers are usually denser than any other layer.
This inspires us to design \ours, where the context is diversely sharded and distributed to each attention head. 
We will discuss the details of our method in the next section.



==> inputs/old_abstract.tex <==

\hao{comments can be hidden by uncommenting line 22 of macros.tex.
you can add your comments with \yuan{} and \suyu{}}
\hao{suggest adding an opening sent reiterating that sparse attn is good, yet their benefits on paper fail to translate to wall-clock ... as in the following sent}
Existing sparse transformer training and inference frameworks struggle in 
bringing wall-clock speed-up while maintaining the model quality.
\hao{i feel that the following statement is a bit too strong. 
i'd reword it and say primarily due to a lack of support of dedicate cuda kernels, sparse attn has yet enjoyed efficiency gain, as canonical attn has from FA. therefore current research is not incentivized to further explore sparse attn}
The line of research thus faded as the thriving of FlashAttention series and risk-averse model architecture choices due to ever-larger training cost.
\hao{we can pack a stronger punch by directly showing off the amount of efficiency gain upfront! so some numbers here would help}
In this paper, we revisit the idea and study how to tame sparsity of self-attention in terms of efficiency and quality in this LLM era.
We design a general and optimized sparse attention kernel library, Sparsely-Sharded (S2) Attention, that allows context-wise, layer-wise, and head-wise customized sparsity patterns.
% To secure coalesced memory access patterns, we implemented a set of tiling and memory layout strategies for sparse computations that balances the system performance and customizability.
\hao{the following 4--5 sentences read too detailed and are hard to follow w/o the context. suggest trimming them. looks like the high-level points we are trying to convey is that our algo. is hardware-aware, and is applicable in various types of sparse attn and in both training and eval}
As attention heads are parallelized in separate thread blocks, the FLOPs reduction in each head could produce end-to-end speed-up and memory reduction over FlashAttention given proper hardware-aware design.
To achieve this, we implemented efficient memory layout strategies like Compressed Sparse Row and corresponding tiling strategies for coalesced memory access.
Also, instead of loading the whole head dimension into SRAM, we split over this dimension to enhance kernel pipelining efficiency.
On the model quality side, we conclude an effective sparse training recipe, context sharding, from experimenting a wide range of sparsity patterns in pre-training, continual pre-training, and inference stages.
The recipe includes three practices to consistently achieve on-par performance with the default self-attention training: (1) diversifying context assignment among attention heads, (2) intact context when union context partitions for each head, (3) inserting a few dense attention layers.
\hao{i feel that the following conclusions are too strong and vague. i'd focus on the actual experiments and results we got}
With large scale of experiments, we show \ours can (1) achieve almost linear speed-up over FlashAttention-2 with respect to theoretical FLOPs reduction, (2) achieve on-par model quality \hao{compared to what?}, especially long context capabilities compared to default attention, (3) linear latency and KV Cache reduction in inference with model quality guarantee. 
We open-sourced \ours and make it compatible with Megatron, Pytorch, and vLLM with a few lines of code.



% Existing LLM training and inference frameworks struggle in 
% boosting efficiency with sparsity while maintaining the integrity of context and model architecture.
% Inspired by the sharding concept in database and the fact that attention parallelizes over heads on accelerators, we propose Sparsely-Sharded (S2) Attention, an attention algorithm that allocates heterogeneous context partitions for different attention heads to divide and conquer.
% \ours\ enforces each attention head to only attend to a partition of contexts following a strided sparsity pattern, while the full context is preserved as the union of all the shards. 
% As attention heads are processed in separate thread blocks, the context reduction for each head can thus produce end-to-end speed-up and memory reduction.
% At inference, LLMs trained with S2-Attention can then take the KV cache reduction as free meals with guaranteed model quality preserve.
% % During inference, LLMs trained with S2-Attention can enjoy the merits of KV cache reduction with guaranteed model quality.
% In experiments, we show \ours can provide as much as (1) 25.3X wall-clock attention speed-up over FlashAttention-2, resulting in 6X reduction in end-to-end training time and 10X inference latency, (2) on-par model training quality compared to default attention, 
% (3)perfect needle retrieval accuracy over 32K context window.
% % (3) better quality preserving compared to post-training sparsification methods.
% On top of the algorithm, we build \repo, an LLM training and inference kernel library that allows users to customize sparsity patterns for their own models. 
% We open-sourced \repo  and make it compatible with Megatron, Pytorch, and vLLM.


==> tables/7btraining.tex <==
\begin{table*}[!h]\centering
\label{tab:7btraining}
\scriptsize
\caption{7B pre-training results. S2 refers to \ours. L refers to number of local blocks. V refers to the vertical stride size.}
\label{tab:7bdownstream}
\begin{tabular}{lrrrrrr}\toprule
Model  & Passkey & MMLU & HellaSwag & WinoGrande & PIQA & Iteration Time(s) \\\midrule
Dense & 1.0 & 0.478 & 0.724 & 0.773 & 0.798 & 4.6\\
S2-L8V15 + Dense & 1.0 & 0.472 & 0.730 & 0.776 & 0.785 & 2.7 \\
\bottomrule
\end{tabular}
\end{table*}

==> tables/head_ab.tex <==
\begin{table*}[!h]\centering
\scriptsize
\caption{7B pre-training results. S2 refers to \ours. L refers to number of local blocks. V refers to the vertical stride size.}
\label{tab:7bdownstream}
\begin{tabular}{lrrr}\toprule
Model  & L8V16 & +Retrieval Head & +2*Retrieval Head\\
\midrule
PPL & 11.72 & 11.61 & 11.61 \\
Passkey & 0.620 & 0.880 & 0.865 \\
\bottomrule
\end{tabular}
\label{tab:headab}
\end{table*}

==> tables/latency.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{End-to-end latency comparison on Llama 1-7B.}
\label{tab:latency}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccc|ccc|cc|c}
\toprule
Batch size &\multicolumn{4}{c|}{1} &\multicolumn{3}{c|}{2} &\multicolumn{2}{c|}{8} &\multicolumn{1}{c}{16} \\
\cmidrule{1-11}
[prompt len, gen len] & \small[32,512] &\small[32,2048] &\small[32,8192] &\small[32,16384] &\small[512,32] &\small[512,512] &\small[4096,4096] &\small[512,512] &\small[4096,4096] &\small[512,512] \\
\midrule
HF &13.35 &57.37 &299 &799.14 &1.12 &19.16 &167.64 &23.44 &OOM &OOM \\
DS &11.58 &47.12 &201.23 &435.74 &0.79 &10.45 &91.04 &12.93 &127.94 &OOM \\
FastGen &11.21 &44.6 &179.43 &359.83 &0.73 &9.71 &76.93 &10.57 &82.16 &OOM \\
Speed-up(\%) over HF &16.03\% &22.30\% &40.00\% &55.00\% &34.80\% &49.30\% &54.10\% &54.90\% &- &OOM \\
Speed-up(\%) over DS &3.20\% &5.35\% &10.83\% &17.42\% &7.59\% &7.08\% &15.50\% &18.25\% &35.78\% &OOM \\
\bottomrule
\end{tabular}
}

\end{table}

==> tables/layer_ab.tex <==
\begin{table*}[!h]\centering
\scriptsize
\caption{Number of dense layers and insertion location Ablation}
\begin{tabular}{lrrrrrrr}\toprule
Model  & L8V16 & +Dense1,2 & +Dense23,24 & +Dense12,13 &  +Dense12,18,24 &  +Dense8,16,24 & +Dense18-24 \\
\midrule
PPL & 11.72 & 11.49 & 11.51 & 11.49 & 11.49 & 11.49 &11.82 \\
Passkey & 0.620 & 0.840 & 0.916 & 0.945 & 0.964 & 0.923 &0.824 \\
\bottomrule
\end{tabular}
\label{tab:layerab}
\end{table*}

==> tables/throughput.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table}[!htp]\centering
\caption{End-to-end latency comparison on Llama 1-7B.}
\label{tab:latency}
\resizebox{\columnwidth}{!}{
\begin{tabular}{l|cccc|ccc|cc|c}
\toprule
Batch size &\multicolumn{4}{c|}{1} &\multicolumn{3}{c|}{2} &\multicolumn{2}{c|}{8} &\multicolumn{1}{c}{16} \\
\cmidrule{1-11}
[prompt len, gen len] & \small[32,512] &\small[32,2048] &\small[32,8192] &\small[32,16384] &\small[512,32] &\small[512,512] &\small[4096,4096] &\small[512,512] &\small[4096,4096] &\small[512,512] \\
\midrule
HF &13.35 &57.37 &299 &799.14 &1.12 &19.16 &167.64 &23.44 &OOM &OOM \\
DS &11.58 &47.12 &201.23 &435.74 &0.79 &10.45 &91.04 &12.93 &127.94 &OOM \\
FastGen &11.21 &44.6 &179.43 &359.83 &0.73 &9.71 &76.93 &10.57 &82.16 &OOM \\
Speed-up(\%) over HF &16.03\% &22.30\% &40.00\% &55.00\% &34.80\% &49.30\% &54.10\% &54.90\% &- &OOM \\
Speed-up(\%) over DS &3.20\% &5.35\% &10.83\% &17.42\% &7.59\% &7.08\% &15.50\% &18.25\% &35.78\% &OOM \\
\bottomrule
\end{tabular}
}

\end{table}
